Searching Mobile App Screens via Text + Doodle

Locating a specific mobile application screen from existing repositories is restricted to basic keyword searches, such as Google Image Search, or necessitates a complete query screen image, as in the case of Swire. However, interactive partial sketch-based solutions like PSDoodle have limitations, including inaccuracy and an inability to consider text appearing on the screen. A potentially effective solution involves implementing a system that provides interactive partial sketching functionality for efficiently structuring user interface elements. Additionally, the system should incorporate text queries to enhance its capabilities further. Our approach, TpD, represents the pioneering effort to enable an iterative search of screens by combining interactive sketching and keyword search techniques. TpD is built on a combination of the Rico repository of approximately 58k Android app screens and the PSDoodle. Our evaluation with third-party software developers showed that PSDoodle provided higher top-10 screen retrieval accuracy than state-of-the-art Swire and required less time to complete a query than other interactive solutions.

==> alt.tex <==
% \CC{These quotes are helpful. The last two I would work into an opening sentence (something like: ``Besides one-word answers (``Great'' and ``Excellent''), users said the following.''}

% \begin{quote}
% ``It was interesting, although some of the drawings did not seem to be recognized.''
% \end{quote}

% \begin{quote}
% ``The idea and the accuracy really amazed me''
% \end{quote}

% \begin{quote}
% ``Great, bit of lag with the refresh, but that's ok''
% \end{quote}

% \begin{quote}
% ``It was interesting, although some of the drawings did not seem to be recognized.''
% \end{quote}

% \begin{quote}
% ``Great''
% \end{quote}

% \begin{quote}
% ``Excellent.''
% \end{quote}

\toolwithtext{} then normalizes the score for a text query and merges it into the final screen score. Finally, \toolwithtext{}'s algorithm combines the scores from the text and sketch search and ranks the mobile screens based on their score, with the highest-scoring screens appearing at the top of the list.

\CC{Few questions:
-- should res-cur be renamed to res? If no, should it be initialized in line 1?}
\CC{-- if user enters one text query of two words, is text in elasticsearch(text) a word or the two-word text?
}
\SM{res\_cur should be initialized within for loop. I have changed the variables. Let me know if it works. Two-word}
\CC{Ok, when we store a two-word text from a corpus screen text in ElasticSearch, do you store it as two one-words (with 3 synonyms each), as one two-word, or both?}
\SM{For any text query, each text tokenized in words and passed to elasticsearch. But I have configured Elasticsearch to do the tokenization. It is not part of algorithm. I have mentioned it in the text }

\toolName{}'s algorithm has five hyperparameters. To ascertain the optimal values for the hyperparameters, \toolName{} collected a total of 30 sketches, which are publicly available online.

Before merging \toolName{}'s score to the final score, \toolwithtext{}'s algorithm normalizes the score to ensure that each sketch element can contribute equally. 

for the three scale levels of search granularity ($p_1$, $p_2$, $p_3$). $\Delta_w$ controls shape, and $C_w$ controls the occurrence difference to match a screen for the doodle type. 

With a change in text set or completion of a drawing, \toolwithtext{} iterates through the search query elements and calculates the score for 58k~Rico screens. Algorithm~\ref{alg:algorithm2} of \toolwithtext{} computes a screen score for every sketch and text query individually. 

-- Storing in ElasticSearch:
    -- Store entire multi-word text phrase
    -- Do not store individual words in addition to phrase
    -- Update a separate mapping from word to 3 synonyms each
    -- Syononym mapping does NOT map multi-word phrase to synonyms
-- res-txt is a dictionary like above
    -- screenID --> screenScore
-- sketch := 2-dim structure
-- doodles := list of icon sketches of same type
-- res-ddl := screenID --> screenScore
-- max(res-ddl) = max of screenScores


% These scores are then normalized and combined for the final screen score. \toolwithtext{} returns the final result by sorting the score in descending order.  

\CC{When storing the (phrase+location --> screenID), do you use the original phrase or a phrase that consists of the pre-processed version of each word in the phrase?}
\SM{Pre-processed version}

-- Table 1
    -- all / last = counts of test icons, e.g., 7/143 camera icons not detected in any stroke
-- Resampling
    -- In a stroke: Find biggest distance between any two line endpoints
    -- Multiply this biggest distance by 20 ==> New nr endpoints

\SM{20 endpoints for 1 unit distance, if the max distance between two endpoints is 2 then 40. }\CC{What is a unit distance?} \SM{Stroke has  endpoints, we find the Euclidian distance of all endpoints, and pick the max distance between those endpoints. Then multiply by 20 to get how many endpoints to represent the current stroke. Add interpolation to find the endpoints  }

-- Resample both
    -- would be harder to convert QD strokes to DoodleUINet
    -- easier to implement resampling of both
    -- Coordinate := X/Y in pixel space
-- Resample stroke :=
    -- Interpolate using NumPy library
        -- used default interpolation style
        -- one-dimensional linear interpolation 
    -- Convert each stroke to have a fixed number of lines
    -- Picked fixed number of lines / stroke 
        -- Used same nr lines / stroke as earlier work in similar domain 
        -- Reference added

Prior research has implemented resampling techniques to mitigate the issue of variation in online writings~\cite{namboodiri2004online}. Our current investigation proposes an alternative approach, wherein we leveraged the NumPy interpolation function - specifically, a one-dimensional linear interpolation - to resample the endpoint coordinates of the strokes. Our pipeline is designed to standardize the number of points for each stroke, irrespective of the drawing interface employed.  \toolwithtext{} added the resampling pipeline in its current implementation to ensure the user drawings have the same sampling ratio.

-- WnD uses exact same DL architecture as PSDoodle
-- QD canvas code was not available
    -- DoodleUINet had different canvas

Training Deep Neural Networks using datasets with varying sampling ratios across categories presents a challenge for learning the underlying structure, which can result in detection accuracy variations across the categories of \QD{} and \dataName{}. 

, which sample endpoint coordinates with different sampling ratios. So for the same stroke, \QD{} and \dataName{} have different numbers of endpoints. 

-- query stack: Order does not matter
    -- rename to ``set of query terms''? -- done
-- exact number != 58,000
    -- rename to 58k -- done

\toolwithtext{}'s install Elasticsearch on the same AWS EC2 to store all preprocessed, curated texts indexed by Rico mobile screen id mapped and mapped with position field. 

also supports queries that differ by a specific Levenshtein edit distance, determining the degree of difference between two sequences. \toolwithtext{} selects a Levenshtein edit distance of 1, allowing for some variation in query submission and minimizing delays for faster results. 

-- Can tell ElasticSearch what is original term and what are its synonyms
    -- hopefully it indexes synonyms just like original word
-- For storing: indexing the document has 4 non-overlapping areas (tl, tr, ..)
-- ElasticSearch feature (``mapping'')
    -- divide document into 4 parts
    -- feature of indexing (document has four fields)
    -- each document (screen) has unique ID
    -- maps (word,zone) to list of document IDs    

\toolwithtext{} configures Elasticsearch to handle the three synonyms generated during screen content expansion. 

tool in the industry that provides fast and real-time data storage, search, and analysis capabilities~\cite{elasticsearch}. Uber, Shopify, and Udemy have adopted Elasticsearch~\cite{elasticsearch,divya_elasticsearch,zamfir_elasticsearch} to enable comprehensive search experiences across large data sets. \toolwithtext{} leverages Elasticsearch to store and index all preprocessed text, facilitating faster retrieval. 

% \CC{What do you do if a screen text has a lot of overlap with 2 quadrants? Do you still map it to only one of them?} \SM{Map according to top-left co-ordinate of the UI element}

\toolwithtext{} then maps the curated text's position on the screen to the 2-by-2 coordinate. \toolwithtext{} then map each text in Elasticsearch with one of the four possible position fields (tl: top-left, tr: top-right, bl: bottom-left, and br: bottom-right). Mapping text with positional fields enables users to label text with its position on the screen, facilitating a more precise and targeted search and yielding more accurate search results.

To enhance spatial awareness, \toolwithtext{} divides the mobile app screen into a 2-by-2  coordinate system, representing the top-left, top-right, bottom-left, and bottom-right corners.

ConceptNet~\cite{conceptnet} maintains a knowledge graph that encodes common sense knowledge (including synonyms, hyponyms, and antonyms) to connect words.  We chose ConceptNet as a knowledge source in our research because of its vast knowledge graph, which boasts over 34 million edges and 5.6 million nodes. Leveraging the strengths of both WordNet and ConceptNet was particularly effective in enabling automatic query expansion\cite{hsu2008combining}.

For instance, WordNet~\cite{Wordnet} indicates that ``picture'' and ``movie'' are synonymous with the term ``film''. Synonyms such as ``picture'', ``movie'', and ``film'' can be used interchangeably in mobile screen content.

such as people's names or places are specific to particular entities, and \toolwithtext{} does not apply AQE to words tagged as named entities. 

-- For each corpus word:
    -- Feed word to 3 contextual models
    -- Each model returns an ordered list of synonym words (with score of each word (0..1))
    -- If word only in one or two contextual models: Just use 10/20 words
    -- If word not in any contextual model:
        -- Get first 3 from WordNet (not scored)
        -- If not in WordNet either: Pick 3 from ConceptNet
    -- Merge all 30, add up scores for each of 30 words
    -- Re-rank 30 words
    -- May need a tie-breaker: 
        -- If one word is not in WordNet then pick other word
        -- So far always one or both in WordNet
        -- If both in WordNet: Decide via ConceptNet
    -- Pick top-3 from re-ranked list
-- WordNet + ConceptNet
    -- Added study and cited it accordingly
    -- If a word has less than 10 synonyms, then fill up with hyponyms
    -- hypernym not used as
    -- Never got to this situation, so always just used synonyms
    -- Ignore order among synonyms, just use them as a set
-- Synonym.txt
    -- 52k screens
    -- some 4 words / screen
    -- NOT 200k words (due to repetition)
    -- We have 36951 words
    -- Remove named 7,448 entities
    -- Total == 29503 * 4 (word + 3 synonyms)
-- Why not expand names?
    -- common in NLP not to do that    
-- Tried fine-tuning of word-embedding with
    -- GloVe + Word2Vec
    -- Not: FastText as library pre-training library does not support it
-- cosine similarity
    -- find words that are used in a similar context as input word    

We used the cosine similarity metric to find similar words in the word embedding because it considers vector orientation and provides better matches than other similarity metrics like Euclidean distance~\cite{mikolov2013efficient}. Afterward, we created a top 10 similar words and their corresponding cosine similarity scores for each model. \toolwithtext{} aggregates the outcomes of the three models based on their scores and then utilizes a majority voting algorithm to ascertain the top three words.

Word2vec model pre-trained on the large corpus word2vec-google-news-300 (100 billion words from the Google News dataset), GloVe pre-trained on glove-wiki-gigaword-300 (Wikipedia 2014 Gigaword, 5.6B tokens, 400K vocab), and FastText pre-trained on fasttext-wiki-news-subwords-300 (a text corpus with more than 9 billion words).  To avoid bias towards the training corpus and capture each model's distinct contexts, \toolwithtext{} combines the output of three-word embedding models.

As training Word Embedding Models on a local corpus fails to capture any meaningful context for a mobile screen text, \toolwithtext{} adopted three pre-trained models for contextual analysis. \toolwithtext{} used Word2vec~\cite{word2vec}, Glove\cite{glove}, andFastText~\cite{fasttext} due to their ability to generate highly accurate word embeddings and capture complex semantic relationships between words. Word2vec~\cite{word2vec}, Glove~\cite{glove}, and FastText~\cite{fasttext} learn the concept of a word by training on a large corpus. 

The text on buttons or other UI elements also briefly describes what each feature does, like ``Afternoon Boost'' or ``Challenge Accepted''. Rico's mobile screen contains an average of four words. Fine-tuning the pre-trained model on brief and discrete descriptions of mobile app features fails to identify any meaningful contextual similarity. In this regard, the Word2vec~\cite{word2vec} model trained on local corpus finds that the terms ``edit'' and ``too'' are the most common terms related to the word ``avatar''. 

(e.g., a given screen's text fragments often represent different app features)

and fine-tuned them using the extracted screen contents. When we use a mobile app, we often see text messages separated into sections and boxes representing different features of the mobile application. 

The contextual analysis involves studying the relationships between words in a vocabulary by examining various features, such as the tendency for related words to appear together in a document. For example, the term ``player'' often occurs in the context of ``sport'', while ``mother'' is frequently associated with ``child''. By analyzing such relationships, contextual analysis can broaden search results by finding related terms. 
 
Automatic Query Expansion (AQE) algorithms improve performance in information retrieval by extending the initial query with additional, relevant terms. Standard

Word embedding is a popular technique used in contextual analysis that represents a word as a dense vector of real numbers, where each vector dimension captures various relationships between phrases. Deep learning methods are trained in an unsupervised manner on large amounts of unstructured text to generate the vector embedding~\cite{word2vec,fasttext}. Through training, word embeddings learn about the context of words within a sentence and identify their semantic relations with other words. Contextually related words tend to be positioned close to each other in the embedding vector space~\cite{word2vec, glove}. Various vector distance measuring metrics, including l1, l2, and cosine, can identify semantically related words which are in close proximity in the embedding space. 

-- Tried OCR to extract text
-- Text extraction := copy paste from JSon that describes screen hierachy
-- Pre-processing of text
    -- only difference is stop word removal
-- Finding names of persons / organization
    -- Language model has that feature built-in
    -- use various methods to determine name / no-name
-- AQE is a common term
    -- others use it to expand query
    -- We do ACE = Automatic Corpus Expansion
    -- Rename to TE := Text Expansion   
-- WordNet was top-choice according to what?
-- ConceptNet: Study that names it


identifies the lemma form of words and stores them in lowercase formats, such as 'energize' for the word 'Energizing.' Additionally, \toolwithtext{} keep track of a text if it is a named entity, such as person names, organizations, and locations.

\toolwithtext{}'s repository includes all these preprocessed extracted texts.

Stemming algorithms, such as Porter~\cite{porter1980algorithm} and Lovin's~\cite{lovins1968development}, use a set of rules to identify the root of a word (e.g., by stripping the suffix from a word ending in ``ed''). The rule-based stemming process cannot recognize the morphological root of a word, as it does not consider the word's part of speech (POS) or its contextual usage within a sentence. Stemming algorithms are also vulnerable where a word's inflected form does not follow any rule (e.g., ``mice'', ``mouse''). 

To ensure retrieval is not affected by any inflectional (e.g., arrive, arrived, arrives) or derivational-related changes (e.g., hopeful, hope), \toolwithtext{} converts each word to its morphological root (e.g., come, comes, came into come), also known as lemmatization. 

Lemmatization algorithms determine the morphological root of a word based on the word's context and part of speech within a sentence, unlike the stemming process. This results in a more precise base form, such as 'bet', or the retention of the original form, such as 'better', depending on the word's POS and context. 

% \CC{Not clear why not used stop word feature in spaCy} \SM{During collection, I have used nltk to remove the stop words.  Later I decided to use spacy for lemmatization. Spacy stop-word implementation is kind of the same as nltk  }
% \CC{Does your pipieline first run stop-word removal or spaCy's lemmatization?}

Stop words ('to,' 'the') appear in high frequency and carry little distinctive information\cite{abadi2016tensorflow}, \toolwithtext{} created a stop-word list using the Natural Language Toolkit~\cite{nltk} and removes them from the curated visible texts. 
\CC{Not clear why not used stop word feature in spaCy}
\CC{Does your pipieline first run stop-word removal or spaCy's lemmatization?}

\toolwithtext{} created its stop-word list using the Natural Language Toolkit~\cite{nltk}.

However, \toolwithtext{} preserves stop-words in the UI element descriptions because words such as ``up'' or ``down''  have distinct features that differentiate one UI element from another (e.g., arrow up, arrow down). \toolwithtext{}'s repository includes all these preprocessed extracted texts.

Text preprocessing is a crucial step to improve natural language processing (NLP) performance in many use cases (e.g., in sentiment analysis, document categorization, and document retrieval for user queries~\cite{manning1999foundations, sebastiani2002machine}). To make the system more robust to text queries, \toolwithtext{} uses two separate text preprocessing pipelines, one for screen text and the other for UI element descriptions. 
% Each pre-processing pipeline consisting of several preprocessing steps.

\toolwithtext{} also extracts all UI element descriptions (e.g., as shown on the right of Figure~\ref{fig:semantic_annotaion}), as they collectively represent all the content displayed on a mobile screen. 

To provide spatial awareness to text query, \toolwithtext{} pulls the absolute position of the text from Rico hierarchy.  

\toolwithtext{} retrieves all the displayed text on a given Rico mobile app screen (as shown on the left of Figure~\ref{fig:semantic_annotaion}) from the hierarchy information, such as ``full body'' and ``absolute calorie''.

\CC{converting an existing (compressed) jpeg to a png does not improve the quality of the image :-). If you zoom in you can see the compression artifacts, which don't look great and make it harder to see what is going on.}
 \SM{The thing is, those mobile screen images are JPEG. Making PNG is not helping much. I will try to fix the issue.}
 \SM{Converted each screen to high res and created this image. Let me know if it is ok. Added another high res with 'hs' extension }

 \CC{I like the general format of this figure. But currently the text query feels like a bit of an after-thought here. The query does not specify the location of the text and there is only one at the end.} \SM{ Created two alternative image }\CC{The alternative images also do not use the lt/tl etc. operators either. The figure shows four queries (query==row). Why not do 2 rows with sketched queries and 2 rows with text queries? At least one of the text queries should contain an position operator. Ideally mix up sketch and text queries (e.g.: sketch, text, sketch, text) or something else besides the current (sketch,sketch,sketch, text).}
\SM{1. Only one query with position syntax. } \CC{If the participants did not use position-text queries, that is not a good sign first of all. Second, do we really have to use a participant query session or can we design our own? Not sure, participant-session would clearly be better. But the current examples do not look that different from PSDoodle, so I am a little worried about ``what is new here'' kind of questions from reviewers.} \SM{I can create an example session with position syntax. the one added right now only has two text and two sketch query from a participant. }

==> seperate_tables.tex <==
% \begin{table}[htbp]
% \begin{center}
%   \caption{Time of participant (P)'s \toolwithtext{} query session to search for a given target screen and iteratively retrieve result screens for each user query. In \toolwithtext{}'s final ranking, the target screen's position~(p) was mostly in the top-10. \CC{It would be good to fit the two Table 2 columns directly before these two columns for all three targets. Even if we have to change the table to full-page-width it would still make it easier to see patterns (currently you have to compare values in two different tables that are on two different pages).}}
%    % in 93\% of cases.
  
%   \label{tab:participantsScorewithtext}
%   \begin{tabular}{r|rr|rr|rr}
%    \hline
%     \multicolumn{1}{c|} {\textbf{P}} &
%     \multicolumn{2}{c|} {\textbf{Target 1}} &
%     \multicolumn{2}{c|} {\textbf{Target 2}} &
%     \multicolumn{2}{c} {\textbf{Target 3}}
%     \\
%     & t[s] & p & t[s] & p & t[s] & p   \\
%       \hline
% 1 & 96 & 4 & 32 & 4 & 71 & 1 \\
% 2 & 12 & 1 & 50 & 29 & 156 & 1 \\
% 3 & 89 & 15 & 23 & 1 & 52 & 2 \\
% 4 & 125 & 1 & 38 & 2 & 19 & 10 \\
% 5 & 15 & 3 & 5 & 3 & 60 & 1 \\
% 6 & 26 & 2 & 38 & 4 & 12 & 7 \\
% 7 & 41 & 1 & 17 & 4 & 18 & 5 \\
% 8 & 90 & 1 & 14 & 7 & 57 & 1 \\
% 9 & 48 & 2 & 28 & 2 & 17 & 4 \\
% 10 & 30 & 1 & 68 & 3 & 18 & 1 \\

%     \hline
% \end{tabular}
% \end{center}
% \end{table}

% \begin{table}[htbp]
% \begin{center}
%   \caption{To retrieve a given Rico target screen using \toolwithtext{}, participant P iteratively issued SQ~sketch queries and TQ~text queries.  }
  
%   \label{tab:participantscombine}
%   \begin{tabular}{r|cc|cc|cc}
%    \hline
%     \multicolumn{1}{l|} {\textbf{P}} &
%     \multicolumn{2}{c|} {\textbf{Target 1}} &
%     \multicolumn{2}{c|} {\textbf{Target 2}} &
%     \multicolumn{2}{c} {\textbf{Target 3}}
%     \\
%     & SQ & TQ & SQ & TQ & SQ & TQ   \\
%       \hline
% 1 & 3 & 1 & 2 & 1 & 3 & 2 \\
% 2 & 2 & 3 & 4 & 1 & 2 & 3 \\
% 3 & 6 & 0 & 2 & 1 & 3 & 0 \\
% 4 & 3 & 1 & 3 & 1 & 3 & 0 \\
% 5 & 2 & 1 & 2 & 1 & 3 & 2 \\
% 6 & 2 & 1 & 3 & 0 & 2 & 1 \\
% 7 & 2 & 1 & 2 & 1 & 2 & 2 \\
% 8 & 2 & 4 & 3 & 2 & 5 & 0 \\
% 9 & 3 & 2 & 2 & 1 & 2 & 1 \\
% 10 & 2 & 1 & 3 & 0 & 3 & 1 \\
%     \hline
% \end{tabular}
% \end{center}
% \end{table}

